An assessment of measuring local levels of homelessness through proxy social media signals

Recent studies suggest social media activity can function as a proxy for measures of state-level public health, detectable through natural language processing. We present results of our efforts to apply this approach to estimate homelessness at the state level throughout the US during the period 2010-2019 and 2022 using a dataset of roughly 1 million geotagged tweets containing the substring ``homeless.'' Correlations between homelessness-related tweet counts and ranked per capita homelessness volume, but not general-population densities, suggest a relationship between the likelihood of Twitter users to personally encounter or observe homelessness in their everyday lives and their likelihood to communicate about it online. An increase to the log-odds of ``homeless'' appearing in an English-language tweet, as well as an acceleration in the increase in average tweet sentiment, suggest that tweets about homelessness are also affected by trends at the nation-scale. Additionally, changes to the lexical content of tweets over time suggest that reversals to the polarity of national or state-level trends may be detectable through an increase in political or service-sector language over the semantics of charity or direct appeals. An analysis of user account type also revealed changes to Twitter-use patterns by accounts authored by individuals versus entities that may provide an additional signal to confirm changes to homelessness density in a given jurisdiction. While a computational approach to social media analysis may provide a low-cost, real-time dataset rich with information about nationwide and localized impacts of homelessness and homelessness policy, we find that practical issues abound, limiting the potential of social media as a proxy to complement other measures of homelessness.

==> paper-template-revtex4.settings.tex <==
\newcommand{\filenamebase}{paper-template}


==> paper-template.biblio.tex <==
\bibliography{\filenamebase}



==> paper-template.contributions.tex <==
Yoshi Bird provided initial motivation for the project and completed statistical analysis of correlations between homelessness and tweet volume, as well as allotaxonometric and user account type analytics. She is also responsible for writing the draft for journal submission. Sarah Grobe queried the Twitter API to generate a full 2010-2022 dataset and preprocessed tweets to provide a clean dataset for analysis. She also completed sentiment analysis and provided statistical and visualization support throughout, as well as post-draft revision and editing support. Michael Arnold provided support with the allotaxonometry and Storywrangler tools, as well as early visualizations. Sean Rogers provided code that accessed Twitter data and structured the results of the query in Pandas objects that were useful for analysis. Mikaela Fudolig and Julia Zimmerman provided feedback on the project as it evolved, as well as revision and editing support post-completion.  


==> paper-template.keywords.tex <==
complex systems,
homelessness,
social media,
Twitter,
computational linguistics,
sentiment analysis


==> paper-template.nutshell.tex <==
Statistically significant nonparametric correlations between homelessness volume and a jurisdiction's rate of tweeting about homelessness, as well as changes to the semantic content of homelessness-related tweets that exist at the national and state level as trends in homelessness volume reverse polarity, suggest that social media data could be useful in detecting real-time changes to homelessness volume, both at a national and a sub-national scale. 


